Open-set Face Recognition for Small Galleries Using Siamese Networks

Face recognition has been one of the most relevant and explored fields of Biometrics. In real-world applications, face recognition methods usually must deal with scenarios where not all probe individuals were seen during the training phase (open-set scenarios). Therefore, open-set face recognition is a subject of increasing interest as it deals with identifying individuals in a space where not all faces are known in advance. This is useful in several applications, such as access authentication, on which only a few individuals that have been previously enrolled in a gallery are allowed. The present work introduces a novel approach towards open-set face recognition focusing on small galleries and in enrollment detection, not identity retrieval. A Siamese Network architecture is proposed to learn a model to detect if a face probe is enrolled in the gallery based on a verification-like approach. Promising results were achieved for small galleries on experiments carried out on Pubfig83, FRGCv1 and LFW datasets. State-of-the-art methods like HFCN and HPLS were outperformed on FRGCv1. Besides, a new evaluation protocol is introduced for experiments in small galleries on LFW.

==> sections/abstract.tex <==
% mostrar no abstract que propos arq
% introduzir em uma ou duas sentencas so
% falar que testou loss function margin
% citar depois
%
\begin{abstract}

Face recognition has been one of the most relevant and explored Biometrics fields. In real-world applications, face recognition methods usually must deal with scenarios where not all probe individuals were seen during training phase (open-set scenarios). 
Therefore, open-set face recognition is a subject of increasing interest as it deals with identifying individuals in a space where not all faces are known in advance.
This is useful in several applications, such as access authentication, on which only a few individuals that have been previously enrolled in a gallery are allowed.
The present work introduces a novel approach towards open-set face recognition focusing on small galleries and in enrollment detection, not identity retrieval.
A Siamese Network architecture is proposed to learn a model to detect if a face probe is enrolled in the gallery based on a verification-like approach.
Promising results were achieved for small galleries, outperforming state-of-the-art methods like HFCN and HPLS, on experiments carried out on Pubfig83, FRGCv1 and LFW datasets. 
In addition, a new evaluation protocol is introduced for experiments in small galleries.
\end{abstract}

%\begin{keywords}
%    Open-set face recognition, siamese networks, face recognition, small galleries.
%\end{keywords}

